ChatIoT: Large Language Model-based Security Assistant for Internet of Things with Retrieval-Augmented Generation

Internet of Things (IoT) has gained widespread popularity, revolutionizing industries and daily life. However, it has also emerged as a prime target for attacks. Numerous efforts have been made to improve IoT security, and substantial IoT security and threat information, such as datasets and reports, have been developed. However, existing research often falls short in leveraging these insights to assist or guide users in harnessing IoT security practices in a clear and actionable way. In this paper, we propose ChatIoT, a large language model (LLM)-based IoT security assistant designed to disseminate IoT security and threat intelligence. By leveraging the versatile property of retrieval-augmented generation (RAG), ChatIoT successfully integrates the advanced language understanding and reasoning capabilities of LLM with fast-evolving IoT security information. Moreover, we develop an end-to-end data processing toolkit to handle heterogeneous datasets. This toolkit converts datasets of various formats into retrievable documents and optimizes chunking strategies for efficient retrieval. Additionally, we define a set of common use case specifications to guide the LLM in generating answers aligned with users' specific needs and expertise levels. Finally, we implement a prototype of ChatIoT and conduct extensive experiments with different LLMs, such as LLaMA3, LLaMA3.1, and GPT-4o. Experimental evaluations demonstrate that ChatIoT can generate more reliable, relevant, and technical in-depth answers for most use cases. When evaluating the answers with LLaMA3:70B, ChatIoT improves the above metrics by over 10% on average, particularly in relevance and technicality, compared to using LLMs alone.

==> Tables/IoT_Vulnerability_chunk.tex <==
\begin{table}[h!]
    \centering
    \caption{Context Precision and Recall of Different Chunking Configurations for VarIoT-Vulnerability.}
    \begin{tabular}{l|c|c}
        \toprule
        \textbf{Chunking Strategy} & \textbf{Context Precision} & \textbf{Context Recall} \\
        \midrule
        character\_500\_50 & 0.8747044916839244 & 0.9059027777684895 \\
        character\_500\_100 & 0.8764172335325398 & 0.9214285714036564 \\
        character\_500\_150 & 0.9166666666304079 & 0.909219858141312 \\
        character\_500\_200 & 0.9288194444063369 & 0.8913832199442743 \\
        \hline
        character\_1000\_50 & 0.9045138888493924 & 0.8674189814728009 \\
        character\_1000\_100 & 0.8826241134545214 & 0.883391203677662 \\
        character\_1000\_150 & 0.8906619385178783 & 0.8972800925596065 \\
        character\_1000\_200 & 0.8914348063176964 & 0.9178240740313658 \\
        \hline
        character\_1500\_50 & 0.8946759259064815 & 0.8820861677684807 \\
        character\_1500\_100 & 0.8282505909946514 & 0.8814236110828993 \\
        character\_1500\_150 & 0.8944444444222506 & 0.8545918367034864 \\
        character\_1500\_200 & 0.8416666666390626 & 0.8645833333126737 \\
        \hline
        character\_2000\_50 & 0.9291383219528629 & 0.8490848720347871 \\
        character\_2000\_100 & 0.9028368794030143 & 0.8352161431735899 \\
        character\_2000\_150 & 0.9131944444041667 & 0.8530936183907272 \\
        character\_2000\_200 & 0.8592536305113435 & 0.8812056737281028 \\
        \midrule
        recursivecharacter\_500\_50 & 0.9812925169635204 & 0.8976352445699385 \\
        \textbf{recursivecharacter\_500\_100} & \textbf{0.986394557794558} & \textbf{0.9733333333176667} \\
        recursivecharacter\_500\_150 & 0.9829931972403061 & 0.9546666666605 \\
        recursivecharacter\_500\_200 & 0.91326530608733 & 0.9346938775489795 \\
        \hline
        recursivecharacter\_1000\_50 & 0.9548611110772572 & 0.8915614478031145 \\
        recursivecharacter\_1000\_100 & 0.9229166666305556 & 0.8971088435297618 \\
        recursivecharacter\_1000\_150 & 0.9163665466132054 & 0.9585034013168368 \\
        recursivecharacter\_1000\_200 & 0.9124999999812501 & 0.9209183673224491 \\
        \hline
        recursivecharacter\_1500\_50 & 0.8928571428329082 & 0.922196969678303 \\
        recursivecharacter\_1500\_100 & 0.8906249999922743 & 0.9124999999638889 \\
        recursivecharacter\_1500\_150 & 0.9131944444187501 & 0.8522108843375851 \\
        recursivecharacter\_1500\_200 & 0.9219858155695037 & 0.8955965909030145 \\
        \hline
        recursivecharacter\_2000\_50 & 0.9131205673523937 & 0.886182598021681 \\
        recursivecharacter\_2000\_100 & 0.8863945577991497 & 0.8817460317309808 \\
        recursivecharacter\_2000\_150 & 0.8611111110913194 & 0.8897569444235244 \\
        recursivecharacter\_2000\_200 & 0.9064625850087585 & 0.9058333333163333 \\
        \midrule
        tokentext\_500\_50 & 0.9357638888650173 & 0.8956916099575963 \\
        tokentext\_500\_100 & 0.901851851823727 & 0.9247685185025464 \\
        tokentext\_500\_150 & 0.929078014162766 & 0.9172453703470197 \\
        tokentext\_500\_200 & 0.9370748298912416 & 0.8970909090889091 \\
        \hline
        tokentext\_1000\_50 & 0.9149305555117189 & 0.9019510581958499 \\
        tokentext\_1000\_100 & 0.8880445795071682 & 0.843380614634604 \\
        tokentext\_1000\_150 & 0.8915906787988349 & 0.8735224586077422 \\
        tokentext\_1000\_200 & 0.8993055555184029 & 0.8831018518407406 \\
        \hline
        tokentext\_1500\_50 & 0.9181547618750744 & 0.8293650793488379 \\
        tokentext\_1500\_100 & 0.9007092198242909 & 0.8310185185053242 \\
        tokentext\_1500\_150 & 0.89115646255 & 0.847539682528516 \\
        tokentext\_1500\_200 & 0.9013350020458699 & 0.8350954069450522 \\
        \hline
        tokentext\_2000\_50 & 0.8986828773961753 & 0.8414351851515046 \\
        tokentext\_2000\_100 & 0.878472222181771 & 0.8654927248626033 \\
        tokentext\_2000\_150 & 0.9164237123158894 & 0.8548752834252834 \\
        tokentext\_2000\_200 & 0.9226190475911309 & 0.8305555555322222 \\
        \bottomrule
    \end{tabular}
\end{table}


==> Tables/OutputLLMEval.tex <==
\begin{table*}[]
    \centering
    \caption{Comparison of \chatiot\ with LLM only method. We implement \chatiot based on LLaMA3:8B, LLaMA3.1:8B, LLaMA3.1:70B, GPT-4o-mini, and GPT-4o, and compare \chatiot\ with the corresponding underlying LLM without being augmented by our retrievers. The evaluator is LLaMA3:70B.}
    \resizebox{\textwidth}{!}{
    \label{tab:outllama}
    \begin{tabular}{c|c|cc|cc|cc|cc|cc}
    \toprule
    \toprule
    \multicolumn{1}{c|}{\multirow{2}{*}{Role}} & \multirow{2}{*}{Metric} & \multicolumn{2}{c|}{LLaMA3:8B} & \multicolumn{2}{c|}{LLaMA3.1:8B} & \multicolumn{2}{c|}{LLaMA3.1:70B} &\multicolumn{2}{c|}{GPT-4o-mini} & \multicolumn{2}{c}{GPT-4o}\\ \cline{3-12} 
    & & \chatiot & LLM & \chatiot & LLM  & \chatiot & LLM  & \chatiot & LLM  & \chatiot & LLM \\
    \midrule
    \multirow{4}{*}{Consumer} &Acc.  & $4.10$ ($+0.11$) & $3.99$ & $4.50$ ($+0.80$) & $3.70$ & $4.40$ ($+0.70$) & $3.70$ & $4.70$ ($+0.80$) & $3.90$ & $4.55$ ($+0.55$) & $4.00$ \\
    &Rel.  & $4.90$ ($+0.65$) & $4.25$ & $4.90$ ($+0.80$) & $4.10$ & $4.90$ ($+0.90$) & $4.00$ & $5.00$ ($+1.00$) & $4.00$ & $4.85$ ($+0.75$) & $4.10$ \\
    &Tec. &  $4.50$ ($+0.47$) & $4.03$ & $4.40$ ($+0.80$)  & $3.60$ & $4.50$ ($+0.70$) & $3.80$ & $4.45$ ($+0.55$) & $3.90$ & $4.40$ ($+0.25$) & $4.15$ \\
    &Fri.  & $4.30$ ($+0.30$) & $4.00$ & $4.70$ ($+0.90$) & $3.80$  & $4.70$ ($+1.00$) & $3.70$ & $4.90$ ($+1.00$) & $3.90$ & $4.80$ ($+0.75$) & $4.05$\\
    \midrule
   \multirow{4}{*}{Security} &Acc.  & $4.30$ ($+0.26$) & $4.04$ & $4.75$ ($+0.67$) & $4.08$ & $4.70$ ($+0.65$) & $4.05$ & $4.85$ ($+1.19$) & $3.66$ & $4.80$ ($+1.29$) & $3.51$ \\
    &Rel.  &  $4.63$ ($+0.33$) & $4.30$ & $4.95$ ($+0.87$) & $4.08$ & $4.93$ ($+0.81$) & $4.12$ & $4.91$ ($+1.21$) & $3.70$ & $4.83$ ($+1.18$) & $3.65$\\
    &Tec. &  $4.47$ ($+0.23$) & $4.24$ & $4.78$ ($+0.79$) & $3.99$ & $4.82$ ($+0.84$) & $3.98$ & $4.89$ ($+1.18$) & $3.71$ & $4.83$ ($+1.18$) & $3.65$\\
    &Fri.  & $4.04$ ($+0.01$) & $4.03$ & $4.02$ ($+0.87$) & $3.15$ &  $4.09$ ($+0.80$) & $3.29$ & $4.92$ ($+1.43$) & $3.49$ & $4.14$ ($+0.61$) & $3.45$\\
    \midrule
    \multirow{4}{*}{Technical} &Acc.  & $4.45$ ($+0.63$) & $3.82$ & $4.45$ ($+0.37$) & $4.08$ & $4.45$ ($+0.37$) & $4.08$ & $4.80$ ($+0.76$) & $4.04$ & $4.85$ ($+0.61$) & $4.24$\\
    &Rel.  & $4.78$ ($+0.73$) & $4.05$ & $4.65$ ($+0.47$) & $4.18$ &  $4.71$ ($+0.51$) & $4.20$ & $4.90$ ($+0.80$) & $4.10$ & $4.88$ ($+0.63$) & $4.25$\\
    &Tec. & $4.59$ ($+0.83$) & $3.76$ & $4.48$ ($+0.29$) & $4.19$ &  $4.55$ ($+0.31$) & $4.24$ & $4.83$ ($+0.68$) & $4.15$ & $4.88$ ($+0.65$) & $4.23$\\
    &Fri.  & $3.92$ ($+0.44$)  & $3.48$ & $4.22$ ($+0.27$) & $3.95$ & $4.13$ ($+0.27$) & $3.86$ & $4.67$ ($+0.62$) & $4.05$ & $4.49$ ($+0.61$) & $3.88$ \\
    \midrule
    \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{0}{Developer}}} &Acc.  & $4.43$ ($+0.63$) & $3.80$ & $4.40$ ($+0.10$) & $4.30$ &  $4.35$ ($-0.14$) & $4.49$ & $4.80$ ($+0.79$) & $4.01$ & $4.75$ ($+0.93$) & $3.82$\\
    &Rel.  & $4.66$ ($+0.83$) & $3.83$ & $4.60$ ($+0.30$) & $4.30$ &  $4.54$ ($+0.02$) & $4.52$ & $4.86$ ($+0.84$) & $4.02$ & $4.81$ ($+0.97$) & $3.84$ \\
    &Tec. & $4.67$ ($+0.62$) & $4.05$ & $4.50$ ($+0.10$) & $4.40$ &  $4.52$ ($-0.01$) & $4.53$ & $4.94$ ($+0.94$) & $4.02$ & $4.86$ ($+0.87$) & $3.99$\\
    &Fri.  & $4.01$ ($+0.09$) & $3.92$ & $3.90$ ($-0.50$) & $4.40$ & $3.96$ ($-0.24$) & $4.30$ & $4.18$ ($+0.48$) & $3.70$ & $4.11$ ($+0.63$) & $3.48$ \\
    \midrule
    \multicolumn{1}{c|}{\multirow{4}{*}{\rotatebox{0}{Trainer}}} &Acc.  & $4.10$ ($-0.14$) & $4.24$ & $4.30$ ($-0.19$) & $4.49$ &  $4.30$ ($-0.31$) & $4.61$ & $4.55$ ($+0.29$) & $4.26$ & $4.40$ ($+0.17$) & $4.23$ \\
    &Rel.  & $4.56$ ($+0.16$) & $4.40$ & $4.40$ ($-0.11$) & $4.51$ &  $4.62$ ($-0.08$) & $4.70$ & $4.64$ ($+0.24$) & $4.40$ & $4.54$ ($+0.39$) & $4.15$ \\
    &Tec. & $4.11$ ($+0.07$) & $4.04$ & $4.42$ ($-0.07$) & $4.49$ & $4.31$ ($-0.23$) & $4.54$ & $4.58$ ($+0.36$) & $4.22$ & $4.53$ ($+0.21$) & $4.32$\\
    &Fri.  & $4.02$ ($-0.03$) & $4.05$ & $4.08$ ($-0.48$) & $4.56$ &  $4.25$ ($-0.40$) & $4.65$ & $4.33$ ($+0.11$) & $4.22$ & $4.46$ ($+0.22$) & $4.24$\\
    \bottomrule
    \bottomrule
    \end{tabular}}
\end{table*}




==> Tables/vulchunk_test.tex <==
\begin{table}[htbp]
\centering
\caption{VARIoT Vulnerabilities: Precision (p) and Recall (r) for Different Chunking Strategies.}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{(Size, Overlap)} & \textbf{Character} & \textbf{RecursiveCharacter} & \textbf{TokenText} \\
\midrule
(500, 50)  & (0.8747, 0.9059) & (0.9813, 0.8976) & (0.9358, 0.8957) \\
(500, 100) & (0.8764, 0.9214) & (0.9864, 0.9733) & (0.9019, 0.9428) \\
(500, 150) & (0.9167, 0.9092) & (0.9830, 0.9547) & (0.9291, 0.9298) \\
(500, 200) & (0.9288, 0.9194) & (0.9133, 0.9347) & (0.9371, 0.8971) \\
\midrule
(1000, 50)  & (0.9045, 0.8674) & (0.9549, 0.8916) & (0.9149, 0.9024) \\
(1000, 100) & (0.8826, 0.8834) & (0.9259, 0.9187) & (0.8808, 0.8434) \\
(1000, 150) & (0.8907, 0.8973) & (0.9164, 0.9585) & (0.8916, 0.8735) \\
(1000, 200) & (0.8914, 0.9178) & (0.9125, 0.9299) & (0.8993, 0.8936) \\
\midrule
(1500, 50)  & (0.8947, 0.8821) & (0.8929, 0.9222) & (0.9182, 0.8294) \\
(1500, 100) & (0.8832, 0.8814) & (0.8894, 0.8817) & (0.8875, 0.8655) \\
(1500, 150) & (0.8944, 0.8546) & (0.9132, 0.8522) & (0.8912, 0.8475) \\
(1500, 200) & (0.8417, 0.8464) & (0.9220, 0.8959) & (0.8929, 0.8033) \\
\midrule
(2000, 50)  & (0.9291, 0.8941) & (0.9131, 0.8862) & (0.8987, 0.8414) \\
(2000, 100) & (0.9028, 0.8352) & (0.8864, 0.8817) & (0.8785, 0.8655) \\
(2000, 150) & (0.9132, 0.8531) & (0.8611, 0.8839) & (0.9164, 0.8543) \\
(2000, 200) & (0.8593, 0.8812) & (0.9065, 0.9058) & (0.9226, 0.8306) \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[htbp]
\centering
\caption{VARIoT Vulnerabilities: Precision (p) and Recall (r) for Different Chunking Strategies.}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{(Size, Overlap)} & \textbf{Character} & \textbf{RecursiveCharacter} & \textbf{TokenText} \\
\midrule
(500, 50)  & (0.8747, 0.9059) & (0.9813, 0.8976) & (0.9358, 0.8957) \\
(500, 100) & (0.8764, 0.9214) & (0.9864, 0.9733) & (0.9019, 0.9428) \\
(500, 150) & (0.9167, 0.9092) & (0.9830, 0.9547) & (0.9291, 0.9298) \\
(500, 200) & (0.9288, 0.9194) & (0.9133, 0.9347) & (0.9371, 0.8971) \\
\midrule
(1000, 50)  & (0.9045, 0.8674) & (0.9549, 0.8916) & (0.9149, 0.9024) \\
(1000, 100) & (0.8826, 0.8834) & (0.9259, 0.9187) & (0.8808, 0.8434) \\
(1000, 150) & (0.8907, 0.8973) & (0.9164, 0.9585) & (0.8916, 0.8735) \\
(1000, 200) & (0.8914, 0.9178) & (0.9125, 0.9299) & (0.8993, 0.8936) \\
\midrule
(1500, 50)  & (0.8947, 0.8821) & (0.8929, 0.9222) & (0.9182, 0.8294) \\
(1500, 100) & (0.8832, 0.8814) & (0.8894, 0.8817) & (0.8875, 0.8655) \\
(1500, 150) & (0.8944, 0.8546) & (0.9132, 0.8522) & (0.8912, 0.8475) \\
(1500, 200) & (0.8417, 0.8464) & (0.9220, 0.8959) & (0.8929, 0.8033) \\
\midrule
(2000, 50)  & (0.9291, 0.8941) & (0.9131, 0.8862) & (0.8987, 0.8414) \\
(2000, 100) & (0.9028, 0.8352) & (0.8864, 0.8817) & (0.8785, 0.8655) \\
(2000, 150) & (0.9132, 0.8531) & (0.8611, 0.8839) & (0.9164, 0.8543) \\
(2000, 200) & (0.8593, 0.8812) & (0.9065, 0.9058) & (0.9226, 0.8306) \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[htbp]
\centering
\caption{VARIoT Vulnerabilities: Precision (p) and Recall (r) for Different Chunking Strategies.}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{(Size, Overlap)} & \textbf{Character} & \textbf{RecursiveCharacter} & \textbf{TokenText} \\
\midrule
(500, 50)  & (0.8747, 0.9059) & (0.9813, 0.8976) & (0.9358, 0.8957) \\
(500, 100) & (0.8764, 0.9214) & (0.9864, 0.9733) & (0.9019, 0.9428) \\
(500, 150) & (0.9167, 0.9092) & (0.9830, 0.9547) & (0.9291, 0.9298) \\
(500, 200) & (0.9288, 0.9194) & (0.9133, 0.9347) & (0.9371, 0.8971) \\
\midrule
(1000, 50)  & (0.9045, 0.8674) & (0.9549, 0.8916) & (0.9149, 0.9024) \\
(1000, 100) & (0.8826, 0.8834) & (0.9259, 0.9187) & (0.8808, 0.8434) \\
(1000, 150) & (0.8907, 0.8973) & (0.9164, 0.9585) & (0.8916, 0.8735) \\
(1000, 200) & (0.8914, 0.9178) & (0.9125, 0.9299) & (0.8993, 0.8936) \\
\midrule
(1500, 50)  & (0.8947, 0.8821) & (0.8929, 0.9222) & (0.9182, 0.8294) \\
(1500, 100) & (0.8832, 0.8814) & (0.8894, 0.8817) & (0.8875, 0.8655) \\
(1500, 150) & (0.8944, 0.8546) & (0.9132, 0.8522) & (0.8912, 0.8475) \\
(1500, 200) & (0.8417, 0.8464) & (0.9220, 0.8959) & (0.8929, 0.8033) \\
\midrule
(2000, 50)  & (0.9291, 0.8941) & (0.9131, 0.8862) & (0.8987, 0.8414) \\
(2000, 100) & (0.9028, 0.8352) & (0.8864, 0.8817) & (0.8785, 0.8655) \\
(2000, 150) & (0.9132, 0.8531) & (0.8611, 0.8839) & (0.9164, 0.8543) \\
(2000, 200) & (0.8593, 0.8812) & (0.9065, 0.9058) & (0.9226, 0.8306) \\
\bottomrule
\end{tabular}
}
\end{table}

\begin{table}[htbp]
\centering
\caption{VARIoT Vulnerabilities: Precision (p) and Recall (r) for Different Chunking Strategies.}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
\textbf{(Size, Overlap)} & \textbf{Character} & \textbf{RecursiveCharacter} & \textbf{TokenText} \\
\midrule
(500, 50)  & (0.8747, 0.9059) & (0.9813, 0.8976) & (0.9358, 0.8957) \\
(500, 100) & (0.8764, 0.9214) & (0.9864, 0.9733) & (0.9019, 0.9428) \\
(500, 150) & (0.9167, 0.9092) & (0.9830, 0.9547) & (0.9291, 0.9298) \\
(500, 200) & (0.9288, 0.9194) & (0.9133, 0.9347) & (0.9371, 0.8971) \\
\midrule
(1000, 50)  & (0.9045, 0.8674) & (0.9549, 0.8916) & (0.9149, 0.9024) \\
(1000, 100) & (0.8826, 0.8834) & (0.9259, 0.9187) & (0.8808, 0.8434) \\
(1000, 150) & (0.8907, 0.8973) & (0.9164, 0.9585) & (0.8916, 0.8735) \\
(1000, 200) & (0.8914, 0.9178) & (0.9125, 0.9299) & (0.8993, 0.8936) \\
\midrule
(1500, 50)  & (0.8947, 0.8821) & (0.8929, 0.9222) & (0.9182, 0.8294) \\
(1500, 100) & (0.8832, 0.8814) & (0.8894, 0.8817) & (0.8875, 0.8655) \\
(1500, 150) & (0.8944, 0.8546) & (0.9132, 0.8522) & (0.8912, 0.8475) \\
(1500, 200) & (0.8417, 0.8464) & (0.9220, 0.8959) & (0.8929, 0.8033) \\
\midrule
(2000, 50)  & (0.9291, 0.8941) & (0.9131, 0.8862) & (0.8987, 0.8414) \\
(2000, 100) & (0.9028, 0.8352) & (0.8864, 0.8817) & (0.8785, 0.8655) \\
(2000, 150) & (0.9132, 0.8531) & (0.8611, 0.8839) & (0.9164, 0.8543) \\
(2000, 200) & (0.8593, 0.8812) & (0.9065, 0.9058) & (0.9226, 0.8306) \\
\bottomrule
\end{tabular}
}
\end{table}

==> refbak <==
@INPROCEEDINGS {llmiotfuz,
author = {J. Wang and L. Yu and X. Luo},
booktitle = {2024 IEEE Symposium on Security and Privacy (SP)},
title = {LLMIF: Augmented Large Language Model for Fuzzing IoT Devices},
year = {2024},
volume = {},
issn = {},
pages = {881-896},
doi = {10.1109/SP54263.2024.00211},
url = {https://doi.ieeecomputersociety.org/10.1109/SP54263.2024.00211},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {may}
}
@inproceedings{yang2023iot,
  title={Iot software vulnerability detection techniques through large language model},
  author={Yang, Yilin},
  booktitle={International Conference on Formal Engineering Methods},
  pages={285--290},
  year={2023},
  organization={Springer}
}
@inproceedings{ma,
author = {Xiaoyue Ma and Lannan Luo and Qiang Zeng},
title = {From One Thousand Pages of Specification to Unveiling Hidden Bugs: Large Language Model Assisted Fuzzing of Matter {IoT} Devices},
booktitle = {33rd USENIX Security Symposium (USENIX Security 24)},
year = {2024},
isbn = {978-1-939133-44-1},
address = {Philadelphia, PA},
pages = {4783--4800},
url = {https://www.usenix.org/conference/usenixsecurity24/presentation/ma-xiaoyue},
publisher = {USENIX Association},
month = aug
}
@article{mo2024iot,
  title={IoT-LM: Large Multisensory Language Models for the Internet of Things},
  author={Mo, Shentong and Salakhutdinov, Russ and Morency, Louis-Philippe and Liang, Paul Pu},
  journal={arXiv preprint arXiv:2407.09801},
  year={2024}
}
@ARTICLE{llmiotcontrol,
  author={Rong, Bo and Rutagemwa, Humphrey},
  journal={IEEE Network}, 
  title={Leveraging Large Language Models for Intelligent Control of 6G Integrated TN-NTN With IoT Service}, 
  year={2024},
  volume={38},
  number={4},
  pages={136-142},
  keywords={6G mobile communication;Task analysis;Internet of Things;Intelligent control;Quality of service;Training data;Large language models},
  doi={10.1109/MNET.2024.3384013}}

@ARTICLE{sokiotllm,
  author={Ferrag, Mohamed Amine and Ndhlovu, Mthandazo and Tihanyi, Norbert and Cordeiro, Lucas C. and Debbah, Merouane and Lestable, Thierry and Thandi, Narinderjit Singh},
  journal={IEEE Access}, 
  title={Revolutionizing Cyber Threat Detection With Large Language Models: A Privacy-Preserving BERT-Based Lightweight Model for IoT/IIoT Devices}, 
  year={2024},
  volume={12},
  number={},
  pages={23733-23750},
  doi={10.1109/ACCESS.2024.3363469}}
@article{meyuhas2024iotlabel,
  title={IoT Device Labeling Using Large Language Models},
  author={Meyuhas, Bar and Bremler-Barr, Anat and Shapira, Tal},
  journal={arXiv preprint arXiv:2403.01586},
  year={2024}
}
@article{deldari2024auditnet,
  title={AuditNet: A Conversational AI-based Security Assistant},
  author={Deldari, Shohreh and Goudarzi, Mohammad and Joshi, Aditya and Shaghaghi, Arash and Finn, Simon and Salim, Flora D and Jha, Sanjay},
  journal={arXiv preprint arXiv:2407.14116},
  year={2024}
}
@article{ji2024sevenllm,
  title={SEvenLLM: Benchmarking, Eliciting, and Enhancing Abilities of Large Language Models in Cyber Threat Intelligence},
  author={Ji, Hangyuan and Yang, Jian and Chai, Linzheng and Wei, Chaoren and Yang, Liqun and Duan, Yunlong and Wang, Yunli and Sun, Tianzhen and Guo, Hongcheng and Li, Tongliang and others},
  journal={arXiv preprint arXiv:2405.03446},
  year={2024}
}
@article{llmtikg,
  title={Llm-tikg: Threat intelligence knowledge graph construction utilizing large language model},
  author={Hu, Yuelin and Zou, Futai and Han, Jiajia and Sun, Xin and Wang, Yilei},
  journal={Computers \& Security},
  volume={145},
  pages={103999},
  year={2024},
  publisher={Elsevier}
}
@article{shafiq2020corrauc,
  title={CorrAUC: a malicious bot-IoT traffic detection method in IoT network using machine-learning techniques},
  author={Shafiq, Muhammad and Tian, Zhihong and Bashir, Ali Kashif and Du, Xiaojiang and Guizani, Mohsen},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={5},
  pages={3242--3254},
  year={2020},
  publisher={IEEE}
}
@article{vasan2020mthael,
  title={MTHAEL: Cross-architecture IoT malware detection based on neural network advanced ensemble learning},
  author={Vasan, Danish and Alazab, Mamoun and Venkatraman, Sitalakshmi and Akram, Junaid and Qin, Zheng},
  journal={IEEE Transactions on Computers},
  volume={69},
  number={11},
  pages={1654--1667},
  year={2020},
  publisher={IEEE}
}
@article{chaganti2022deep,
  title={Deep learning based cross architecture internet of things malware detection and classification},
  author={Chaganti, Rajasekhar and Ravi, Vinayakumar and Pham, Tuan D},
  journal={Computers \& Security},
  volume={120},
  pages={102779},
  year={2022},
  publisher={Elsevier}
}
@article{otoum2022dl,
  title={DL-IDS: a deep learning--based intrusion detection framework for securing IoT},
  author={Otoum, Yazan and Liu, Dandan and Nayak, Amiya},
  journal={Transactions on Emerging Telecommunications Technologies},
  volume={33},
  number={3},
  pages={e3803},
  year={2022},
  publisher={Wiley Online Library}
}
@inproceedings{aung2022atlas,
  title={ATLAS: A Practical Attack Detection and Live Malware Analysis System for IoT Threat Intelligence},
  author={Aung, Yan Lin and Ochoa, Mart{\'\i}n and Zhou, Jianying},
  booktitle={International Conference on Information Security},
  pages={319--338},
  year={2022},
  organization={Springer}
}
@inproceedings{tambe2019detection,
  title={Detection of threats to IoT devices using scalable VPN-forwarded honeypots},
  author={Tambe, Amit and Aung, Yan Lin and Sridharan, Ragav and Ochoa, Mart{\'\i}n and Tippenhauer, Nils Ole and Shabtai, Asaf and Elovici, Yuval},
  booktitle={Proceedings of the Ninth ACM Conference on Data and Application Security and Privacy},
  pages={85--96},
  year={2019}
}
@article{es2023ragas,
  title={Ragas: Automated evaluation of retrieval augmented generation},
  author={Es, Shahul and James, Jithin and Espinosa-Anke, Luis and Schockaert, Steven},
  journal={arXiv preprint arXiv:2309.15217},
  year={2023}
}
@inproceedings{iacovazzi2023towards,
  title={Towards Cyber Threat Intelligence for the IoT},
  author={Iacovazzi, Alfonso and Wang, Han and Butun, Ismail and Raza, Shahid},
  booktitle={2023 19th International Conference on Distributed Computing in Smart Systems and the Internet of Things (DCOSS-IoT)},
  pages={483--490},
  year={2023},
  organization={IEEE}
}
@book{bou2020cyber,
  title={Cyber threat intelligence for the internet of things},
  author={Bou-Harb, Elias and Neshenko, Nataliia},
  year={2020},
  publisher={Springer}
}
@article{wagner2019cyber,
  title={Cyber threat intelligence sharing: Survey and research directions},
  author={Wagner, Thomas D and Mahbub, Khaled and Palomar, Esther and Abdallah, Ali E},
  journal={Computers \& Security},
  volume={87},
  pages={101589},
  year={2019},
  publisher={Elsevier}
}


@article{al2020survey,
  title={A survey of machine and deep learning methods for internet of things (IoT) security},
  author={Al-Garadi, Mohammed Ali and Mohamed, Amr and Al-Ali, Abdulla Khalid and Du, Xiaojiang and Ali, Ihsan and Guizani, Mohsen},
  journal={IEEE communications surveys \& tutorials},
  volume={22},
  number={3},
  pages={1646--1685},
  year={2020},
  publisher={IEEE}
}

@article{neshenko2019demystifying,
  title={Demystifying IoT security: An exhaustive survey on IoT vulnerabilities and a first empirical look on Internet-scale IoT exploitations},
  author={Neshenko, Nataliia and Bou-Harb, Elias and Crichigno, Jorge and Kaddoum, Georges and Ghani, Nasir},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={21},
  number={3},
  pages={2702--2733},
  year={2019},
  publisher={IEEE}
}

@inproceedings{luo2022transformer,
  title={Transformer-based malicious traffic detection for Internet of Things},
  author={Luo, Yantian and Chen, Xu and Ge, Ning and Feng, Wei and Lu, Jianhua},
  booktitle={ICC 2022-IEEE International Conference on Communications},
  pages={4187--4192},
  year={2022},
  organization={IEEE}
}

@inproceedings{ferraris2024ici,
title = {Enhancing TrUStAPIS Methodology in the Web of Things with LLM-generated IoT Trust Semantics},
author = {Davide Ferraris and Konstantinos Kotis and Christos Kalloniatis},
url = {/wp-content/papers/ferraris2024ici.pdf},
year = {2024},
date = {2024-12-31},
urldate = {2024-12-31},
booktitle = {26th International Conference on Information and Communications Security (ICICS 2024)},
publisher = {Springer},
address = {Mytilene, Lesvos, Greece}
}
@article{kouicem2018internet,
  title={Internet of things security: A top-down survey},
  author={Kouicem, Djamel Eddine and Bouabdallah, Abdelmadjid and Lakhlef, Hicham},
  journal={Computer Networks},
  volume={141},
  pages={199--221},
  year={2018},
  publisher={Elsevier}
}
@article{ahmad2021machine,
  title={Machine learning approaches to IoT security: A systematic literature review},
  author={Ahmad, Rasheed and Alsmadi, Izzat},
  journal={Internet of Things},
  volume={14},
  pages={100365},
  year={2021},
  publisher={Elsevier}
}
@article{mosenia2016comprehensive,
  title={A comprehensive study of security of internet-of-things},
  author={Mosenia, Arsalan and Jha, Niraj K},
  journal={IEEE Transactions on emerging topics in computing},
  volume={5},
  number={4},
  pages={586--602},
  year={2016},
  publisher={IEEE}
}
@article{gormucs2018security,
  title={Security for the internet of things: a survey of existing mechanisms, protocols and open research issues},
  author={G{\"o}rm{\"u}{\c{s}}, Sedat and Ayd{\i}n, Hakan and Uluta{\c{s}}, G{\"u}zin},
  journal={Journal of the Faculty of Engineering and Architecture of Gazi University},
  volume={33},
  number={4},
  pages={1247--1272},
  year={2018}
}
@inproceedings{williams2017identifying,
  title={Identifying vulnerabilities of consumer Internet of Things (IoT) devices: A scalable approach},
  author={Williams, Ryan and McMahon, Emma and Samtani, Sagar and Patton, Mark and Chen, Hsinchun},
  booktitle={2017 IEEE International Conference on Intelligence and Security Informatics (ISI)},
  pages={179--181},
  year={2017},
  organization={IEEE}
}
@inproceedings{deogirikar2017security,
  title={Security attacks in IoT: A survey},
  author={Deogirikar, Jyoti and Vidhate, Amarsinh},
  booktitle={2017 International Conference on I-SMAC (IoT in Social, Mobile, Analytics and Cloud)(I-SMAC)},
  pages={32--37},
  year={2017},
  organization={IEEE}
}
@Article{VARIoT_db,
AUTHOR = {Janiszewski, Marek and Felkner, Anna and Lewandowski, Piotr and Rytel, Marcin and Romanowski, Hubert},
TITLE = {Automatic Actionable Information Processing and Trust Management towards Safer Internet of Things},
JOURNAL = {Sensors},
VOLUME = {21},
YEAR = {2021},
NUMBER = {13},
ARTICLE-NUMBER = {4359},
URL = {https://www.mdpi.com/1424-8220/21/13/4359},
PubMedID = {34202248},
ISSN = {1424-8220},
DOI = {10.3390/s21134359}
}
@incollection{strom2018mitre,
  title={Mitre att\&ck: Design and philosophy},
  author={Strom, Blake E and Applebaum, Andy and Miller, Doug P and Nickels, Kathryn C and Pennington, Adam G and Thomas, Cody B},
  booktitle={Technical report},
  year={2018},
  publisher={The MITRE Corporation}
}

@misc{CVE_Mission,
  author       = {{CVE Program}},
  title        = {{CVE\textsuperscript{\textregistered} Program Mission}},
  year         = {n.d.},
  howpublished = {\url{https://www.cve.org/}}
}
@article{abdul2019comprehensive,
  title={A comprehensive study of security and privacy guidelines, threats, and countermeasures: An IoT perspective},
  author={Abdul-Ghani, Hezam Akram and Konstantas, Dimitri},
  journal={Journal of Sensor and Actuator Networks},
  volume={8},
  number={2},
  pages={22},
  year={2019},
  publisher={MDPI}
}
@article{wright2022regulating,
  title={Regulating to Protect Security and Privacy in the Internet of Things (IoT): Draft Report},
  author={Wright, E and Lindsay, D and Wilkinson, G},
  year={2022},
  publisher={UTS}
}
@article{saurabh2024hms,
  title={HMS-IDS: Threat Intelligence Integration for Zero-Day Exploits and Advanced Persistent Threats in IIoT},
  author={Saurabh, Kumar and Sharma, Vaidik and Singh, Uphar and Khondoker, Rahamatullah and Vyas, Ranjana and Vyas, OP},
  journal={Arabian Journal for Science and Engineering},
  pages={1--21},
  year={2024},
  publisher={Springer}
}
@article{ahmed2023securing,
  title={Securing the Internet of Things (IoT): A comprehensive study on the intersection of cybersecurity, privacy, and connectivity in the IoT ecosystem},
  author={Ahmed, Sarah and Khan, Muhammad},
  journal={AI, IoT and the Fourth Industrial Revolution Review},
  volume={13},
  number={9},
  pages={1--17},
  year={2023}
}
@inproceedings{alrawi2021circle,
  title={The Circle of life: A $\{$large-scale$\}$ study of the $\{$IoT$\}$ malware lifecycle},
  author={Alrawi, Omar and Lever, Charles and Valakuzhy, Kevin and Snow, Kevin and Monrose, Fabian and Antonakakis, Manos and others},
  booktitle={30th USENIX Security Symposium (USENIX Security 21)},
  pages={3505--3522},
  year={2021}
}
@inproceedings{dragomir2016survey,
  title={A survey on secure communication protocols for IoT systems},
  author={Dragomir, Dan and Gheorghe, Laura and Costea, Sergiu and Radovici, Alexandru},
  booktitle={2016 international workshop on Secure Internet of Things (SIoT)},
  pages={47--62},
  year={2016},
  organization={IEEE}
}
@article{gpt,
  title={Improving Language Understanding by Generative Pre-Training},
  author={Alec Radford and Karthik Narasimhan},
  year={2018}
}
@inproceedings{zhuge2021kaleido,
  title={Kaleido-bert: Vision-language pre-training on fashion domain},
  author={Zhuge, Mingchen and Gao, Dehong and Fan, Deng-Ping and Jin, Linbo and Chen, Ben and Zhou, Haoming and Qiu, Minghui and Shao, Ling},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12647--12657},
  year={2021}
}
@inproceedings{docformer,
  title={Docformer: End-to-end transformer for document understanding},
  author={Appalaraju, Srikar and Jasani, Bhavan and Kota, Bhargava Urala and Xie, Yusheng and Manmatha, R},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={993--1003},
  year={2021}
}
@inproceedings{kim2022ocr,
  title={Ocr-free document understanding transformer},
  author={Kim, Geewook and Hong, Teakgyu and Yim, Moonbin and Nam, JeongYeon and Park, Jinyoung and Yim, Jinyeong and Hwang, Wonseok and Yun, Sangdoo and Han, Dongyoon and Park, Seunghyun},
  booktitle={European Conference on Computer Vision},
  pages={498--517},
  year={2022},
  organization={Springer}
}
@misc{chatgpt,
      title={Language Models are Few-Shot Learners}, 
      author={Tom B. Brown and Benjamin Mann and Nick Ryder and Melanie Subbiah and Jared Kaplan and Prafulla Dhariwal and Arvind Neelakantan and Pranav Shyam and Girish Sastry and Amanda Askell and Sandhini Agarwal and Ariel Herbert-Voss and Gretchen Krueger and Tom Henighan and Rewon Child and Aditya Ramesh and Daniel M. Ziegler and Jeffrey Wu and Clemens Winter and Christopher Hesse and Mark Chen and Eric Sigler and Mateusz Litwin and Scott Gray and Benjamin Chess and Jack Clark and Christopher Berner and Sam McCandlish and Alec Radford and Ilya Sutskever and Dario Amodei},
      year={2020},
      eprint={2005.14165},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}
@inproceedings{islam2024gemini,
  title={Gemini-the most powerful LLM: Myth or Truth},
  author={Islam, Raisa and Ahmed, Imtiaz},
  booktitle={2024 5th Information Communication Technologies Conference (ICTC)},
  pages={303--308},
  year={2024},
  organization={IEEE}
}

@inproceedings{fan2024survey,
  title={A survey on rag meeting llms: Towards retrieval-augmented large language models},
  author={Fan, Wenqi and Ding, Yujuan and Ning, Liangbo and Wang, Shijie and Li, Hengyun and Yin, Dawei and Chua, Tat-Seng and Li, Qing},
  booktitle={Proceedings of the 30th ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  pages={6491--6501},
  year={2024}
}
@article{lewis2020retrieval,
  title={Retrieval-augmented generation for knowledge-intensive nlp tasks},
  author={Lewis, Patrick and Perez, Ethan and Piktus, Aleksandra and Petroni, Fabio and Karpukhin, Vladimir and Goyal, Naman and K{\"u}ttler, Heinrich and Lewis, Mike and Yih, Wen-tau and Rockt{\"a}schel, Tim and others},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={9459--9474},
  year={2020}
}
@article{cui2024llmind,
  title={LLMind: Orchestrating AI and IoT with LLM for Complex Task Execution},
  author={Cui, Hongwei and Du, Yuyang and Yang, Qun and Shao, Yulin and Liew, Soung Chang},
  journal={IEEE Communications Magazine},
  year={2024},
  publisher={IEEE}
}
@article{ferraris2020trustapis,
  title={TrUStAPIS: a trust requirements elicitation method for IoT},
  author={Ferraris, Davide and Fernandez-Gago, Carmen},
  journal={International Journal of Information Security},
  volume={19},
  number={1},
  pages={111--127},
  year={2020},
  publisher={Springer}
}
@misc{LLaMA,
title = {LLaMA: Open and Honest},
author = {Jason Wei and Yi Tay and Ruiqi Zhong and Jiaao Chen and Siyuan Wang and Zhengxiang Wang and Boxin Wang and Tengxu Sun and Min Lin and Jennifer Power and Zongwei Zhou and others},
year = {2022},
publisher = {Meta},
url = {\url{https://www.llama.com/}}
}
@inproceedings{xu2024penetrative,
  title={Penetrative ai: Making llms comprehend the physical world},
  author={Xu, Huatao and Han, Liying and Yang, Qirui and Li, Mo and Srivastava, Mani},
  booktitle={Proceedings of the 25th International Workshop on Mobile Computing Systems and Applications},
  pages={1--7},
  year={2024}
}

@misc{ollama2024,
  title = {Ollama},
  note = {Version 0.3.9},
  year = {2024},
  howpublished = {\url{https://github.com/ollama/ollama}} 
}
@article{roziere2023code,
  title={Code llama: Open foundation models for code},
  author={Roziere, Baptiste and Gehring, Jonas and Gloeckle, Fabian and Sootla, Sten and Gat, Itai and Tan, Xiaoqing Ellen and Adi, Yossi and Liu, Jingyu and Sauvestre, Romain and Remez, Tal and others},
  journal={arXiv preprint arXiv:2308.12950},
  year={2023}
}

@misc{liu2024llavanext,
    title={LLaVA-NeXT: Improved reasoning, OCR, and world knowledge},
    url={https://llava-vl.github.io/blog/2024-01-30-llava-next/},
    author={Liu, Haotian and Li, Chunyuan and Li, Yuheng and Li, Bo and Zhang, Yuanhan and Shen, Sheng and Lee, Yong Jae},
    month={January},
    year={2024}
}

@misc{iotnews1,
    title={State of the IoT 2020: 12 billion IoT connections, surpassing non-IoT for the first time},
    url={https://iot-analytics.com/state-of-the-iot-2020-12-billion-iot-connections-surpassing-non-iot-for-the-first-time/},
    author={Knud Lasse Lueth},
    month={November},
    year={2020}
}

@misc{liu2023improvedllava,
      title={Improved Baselines with Visual Instruction Tuning}, 
      author={Liu, Haotian and Li, Chunyuan and Li, Yuheng and Lee, Yong Jae},
      publisher={arXiv:2310.03744},
      year={2023},
}

@misc{liu2023llava,
      title={Visual Instruction Tuning}, 
      author={Liu, Haotian and Li, Chunyuan and Wu, Qingyang and Lee, Yong Jae},
      publisher={NeurIPS},
      year={2023},
}

@article{elasticsearch2018elasticsearch,
  title={Elasticsearch},
  journal={software, version},
  volume={6},
  number={1},
  year={2018}
}

@misc{docker-desktop,
  title = {Docker Desktop, Version 4.29.0},
  year = {2024},
  howpublished = {\url{https://www.docker.com/products/docker-desktop}},
}

@misc{langchain2024,
  title = {LangChain},
  year = {2024},
  howpublished = {\url{https://github.com/langchain-ai/langchain}},
  note = {Version 0.2.5}
}

@misc{streamlit,
  title = {Streamlit, Version 1.33.0},
  year = {2024},
  howpublished = {\url{https://streamlit.io}},
  note = {Accessed: 2024-09-02}
}

